Think Big, Generate Quick: LLM-to-SLM for Fast Autoregressive Decoding

Large language models (LLMs) have become ubiquitous in practice and are widely used for generation tasks such as translation, summarization and instruction following. However, their enormous size and reliance on autoregressive decoding increase deployment costs and complicate their use in latency-critical applications. In this work, we propose a hybrid approach that combines language models of different sizes to increase the efficiency of autoregressive decoding while maintaining high performance. Our method utilizes a pretrained frozen LLM that encodes all prompt tokens once in parallel, and uses the resulting representations to condition and guide a small language model (SLM), which then generates the response more efficiently. We investigate the combination of encoder-decoder LLMs with both encoder-decoder and decoder-only SLMs from different model families and only require fine-tuning of the SLM. Experiments with various benchmarks show substantial speedups of up to $4\times$, with minor performance penalties of $1-2\%$ for translation and summarization tasks compared to the LLM.

==> ethics.text/appendices.tex <==
\clearpage
\setcounter{section}{0}
\section*{Appendix}


\section{PEFT hyperparameters}
\label{sec:peft_hyperparam}
\hyperref[table:peft_hyperparam]{Table~\ref{table:peft_hyperparam}} presents the hyperparameters for the prompt tuning, prefix tuning, and LoRA methods we considered in the parameter-efficient fine-tuning ablation in our paper.

\begin{table}[hbt!]
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{lll}
\toprule
\belowrulesepcolor{my-gray}
\rowcolor{my-gray}
& \textbf{GPT2} & \textbf{T5 Small}\\
\aboverulesepcolor{my-gray}
\midrule
\textbf{Prompt tuning} & &  \\
\# prompt tokens & 200 & 1024\\
\midrule
%\belowrulesepcolor{my-gray}
%\rowcolor{my-gray}
%& \textbf{GPT2} & \textbf{T5 Small}\\
\textbf{Prefix tuning} & & \\
\# prefix tokens & 256 & 1024\\
project. hidden size & 64 & 64\\
\midrule
%\belowrulesepcolor{my-gray}
%\rowcolor{my-gray}
\textbf{LoRA} & & \\
Rank & 40 & 24\\
$\alpha$ & 64 & 32\\
Dropout & 0.1 & 0.1\\
\bottomrule
\end{tabular}
}
\caption{Hyperparameters for prompt tuning, prefix tuning and LoRA.}
\label{table:peft_hyperparam}
\end{table}

\section{Using decoder-only models as LLM}
\label{sec:appendix_decoder_only}
We present preliminary result for using decode-only models as an LLM in our \methodname{} framework on the summarization task. We use GPT2 XL as the LLM and GPT2 base as the SLM in our experiments. Compared to Encoder-Decoder based LLMs, there is no specific layer in the model which can explicitly be identified as the encoded representation of the prompt. Therefore, we experiment with extracting representations from different layers of the GPT XL model before passing it to the projector and subsequently to the SLM. The results are presented in \hyperref[tab:summarization_decoder]{Table~\ref{tab:summarization_decoder}}. Surprisingly, we observe that

\begin{table}[hbt!]
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{llllll}
\toprule
\textbf{Model} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{Avg.}\\
\midrule
GPT2-XL & 40.47 & 19.09 & 28.90 & 29.49 \\ %37.94  \\
GPT2 & 38.58 & 17.56 & 27.36 & 27.83 \\ %36.06 \\
\midrule
GPT2-XL-2-GPT2 (layer 0) & 39.16 & 17.71 & 27.43 & 36.55 \\ %37.64\\
GPT2-XL-2-GPT2 (layer 1) & 39.05 & 17.63 & 27.40 & 36.43 \\ %37.64\\
GPT2-XL-2-GPT2 (layer 4) & 36.66 & 16.46 & 25.64 & 34.87 \\ %37.64\\
GPT2-XL-2-GPT2 (layer 8) & 33.27 & 14.03 & 23.24 & 30.98 \\ %37.64\\
GPT2-XL-2-GPT2 (all layers, weighted avg) & 37.69 & 16.72 & 26.41 & 35.15 \\ %37.64\\\textbf{}
\aboverulesepcolor{my-blue}
%\textcolor{red}{GPT2-XL-2-GPT2} & . & . & . & .\\
\bottomrule
\end{tabular}
}
\caption{ROUGE scores (abbreviated with R-) on CNN/Daily Mail. GPT2-XL (zero-shot) results are from~\citet{radford2019language}. Runtimes are reported in seconds for 100 generated tokens. \color{red}{TODO: Add proper averaging instead of R-AVG}}
\label{tab:summarization_decoder}
\end{table}

\section{MT-Bench qualitative evaluation}
In this section, we present sample qualitative responses by the baseline LLM, SLM, and our proposed \methodname{} on MT-Bench and their corresponding ratings provided by GPT-4 as the judge.
\label{sec:appendix_mtbench}

\input{tables/MTBenchQualitative}







==> ethics.text/conclusions.tex <==
% reflection on results
In this work, we present \methodname{}, a novel framework to speed up autoregressive decoding.
Our approach uses an LLM to encode a prompt for conditioning of an SLM, which then efficiently decodes the response.
Our experiments across various benchmarks demonstrate substantial speedups between $2-4\times$, which are often accompanied by minimal performance penalties between $1-2\%$.

\textcolor{red}{limitations now excluded. Need to revisit conclusions. If you have ideas, feel free to write.}

Other exciting future avenues include further scaling the components of \methodname{}, fine-tuning the LLM together with the SLM, and integrating our method for the design of new efficient architectures.



%We demonstrate that LLM-2-SLM in challengingFor challenging tasks

%Notably, the performance in more challenging setups falls short of the desired level. However, our study also reveals that the combination of our method with Self-Distillation (SD) can ameliorate this limitation, providing a pathway for improved performance in demanding scenarios.

%In conclusion, this paper introduces the \methodname{} framework, a novel approach aimed at accelerating autoregressive decoding through the integration of a Language Model (LLM) to encode prompts for the conditioning of a more efficient Sequence-Level Model (SLM). Our experimental results across various benchmarks demonstrate significant speed-ups, often accompanied by minimal performance penalties, highlighting the effectiveness of our proposed methodology.


% Our experiments across benchmarks show large speed ups up, often at low performance penalty.
% limitations
% performance in more challenging setup not as good. we show that our method together with SD can help in this setting.
% A current limitation of this work is that our approach works well only for bi-directional encoders but not for decoder-only models, as  shown in App X. 
% future work
% Many ways to explore from here:
% train the LLM
% make it work for decoder-only LLM
% further increase scale, in both models.
% real-world application


==> ethics.text/experiments.tex <==
We empirically evaluate the efficacy of our proposed \methodname{} on three tasks: machine translation, summarization, and instruction-tuning. In all our experiments, we intend to answer the following question: What is the comparative performance and runtime of LLM-2-SLM in relation to LLM and SLM alone? %For both metrics, we use the LLM and SLM as baselines and consider them as upper and lower bounds, respectively.

\paragraph{Setup}
%\ya{here you can add the other implementation details}
% We study our method in three different domains and evaluation regimes: traditional fine-tuning on machine translation and abstractive summarization, as well as instruction tuning on various held-out tasks.
The networks used in our experiments are listed in \hyperref[table:models]{Table~\ref{table:models}}.
We employ various pretrained models and transformer architectures and denote specific combinations as LLM$\,\to\,$SLM.
Specifically, we make use of T5 encoders as LLMs, and employ T5 encoder-decoder and GPT2 decoder-only models as SLMs.
%of LLM-2-SLM by substitution, e.g.: T5-Large-2-T5-Small, where T5-Large acts as LLM and T5-Small as SLM.
Our LLMs have $8-55\times$ more parameters than the SLMs.
For generation, we use beam search (beam width of 4, length penalty $\alpha=0.6$) for translation and summarization, and nucleus sampling for instruction tuning.

We report task-specific performance metrics, including SacreBLEU~\cite{post-2018-call} for translation, ROUGE~\cite{lin2004rouge} for summarization and GPT4 as a judge for instruction tuning, using % with the default prompt for single answer grading and 
the same generation settings as~\cite{zheng2023judging}.
Furthermore, we report runtimes, exemplary for 100 generated tokens using either a V100 (translation, summarization) or A100 (instruction tuning) GPU.

\input{tables/model_variants}


\paragraph{Training}
Knowledge distillation~\cite{hinton2015distilling, zhou2023distillspec}, wherein a small student model is trained with the help of a larger teacher model, has been shown to be an effective training strategy to improve the performance of the student network.
This technique is particularly relevant to our method, given the direct connection between the small and large models in our framework.
Therefore, we perform experiments in which we learn either from the ground truth signal provided by a dataset or from sequences generated by the LLM.
All models are trained with cross-entropy loss, AdamW optimizer~\cite{loshchilov2017decoupled} with weight decay of 0.1, learning rate of $0.001$ with linear warmup~\cite{goyal2017accurate} for $10\%$ of the total number of iterations, followed by cosine learning rate decay to $0$~\cite{loshchilov2016sgdr}.
We rely on Huggingface's transformers~\cite{wolf2019huggingface} for training and generation.


%%Learning from GT and distilled representations 

%Optimizer

%huggingface pretrained models

% Research questions

% upper/lower bound

%we denote our models like so: T5-Large-2-T5-Small

%model size comparison:

%training time: specific to datasets

%generation parameters: beam search

%\subsection{Training setup}

\input{tables/translation}
\subsection{Machine translation}

We study our method in translation from English into German, French, and Romanian.
We utilize WMT14~\cite{bojar2014findings} for En-Fr/De, and WMT16 for En-Ro~\cite{bojar2016findings}.
T5 Large serves as LLM and T5 Small, T5 1.1 Small, and GPT2 as SLMs.
T5 Small and GPT2 are $16\times$ and $8\times$ smaller than T5 Large. 
Both T5 Large/Small are pretrained for translation, while T5 1.1 Small was only trained on the C4 dataset.
The following task description precedes the prompt: "\texttt{translate English to *target-language*:}".
All models, except the LLM which is applied directly (called zero-shot), are trained for $50k$ iterations on the train sets and evaluated on the test splits.
We use T5 Large to generate sequences to distill from and report BLEU scores in \hyperref[tab:translation]{Table~\ref{tab:translation}}. %TODO: which BLEU score, Sacrebleu as in t5 paper?
%we use distillation, since it works better.
%T5-Large is X times larger than SLMs.

%The difference in performance between T5 Large and T5 Small is more than $2$ BLEU points for En-Fr and En-De, and $1$ point for En-Ro.
T5 Large shows an average score of $31.94$, while T5 Small performs $2$ BLEU points worse.
fine-tuned SLMs that have not been pretrained for translation perform more than $3$ BLEU points worse than the LLM.
Our LLM-2-SLM variants often reduce these gaps to less than 1 point and come close to the performance of the LLM.
For example, T5 Large$\,\to\,$T5 Small achieves on average $0.4$ points less than the LLM, corresponding to a performance gap of only $1\%$.
Gains over the SLM alone are more pronounced in non-task-pretrained networks, e.g., T5 Large$\,\to\,$T5 1.1 Small scores on average $2.5$ points better than T5 1.1 Small.
Despite having different model families, we also see big gains in T5 Large$\,\to\,$GPT2.
Furthermore, we observe that the significant performance improvements of LLM-2-SLM over SLM come at a marginal trade-off in runtime, which is already evident for short generation lengths (e.g., 100 tokens).
%Moreover, these benefits are already evident for short generation lengths (e.g., 100 tokens).%\textcolor{red}{\hyperref[fig:runtime]{Figure~\ref{fig:runtime}}} presents the runtime comparison between different models.


%Figure~\ref{fig:runtime} shows the relationship between results and V100 GPU runtime. LLM-2-SLM exhibits relative performance gains over SLMs with a slight increase in runtime. These benefits are noticeable even for short generation lengths (e.g., 100 tokens).

%perform substantially better than the SLM alone, while being only slightly slower. These advantages are already evident in settings where the sequence length to be generated is relatively small (e.g., 100 tokens).
% difference between T5-Large and T5-Small is more than two points better for French and German, and ca. one point better for Romanian.
%fine-tuned SLMs not pretrained for translation are ca. 2-4 points worse than the LLM.
%Our LLM-2-SLM variants reduce these gaps often times below 1 point and approach the performance of the LLM. For example, T5-Large-2-T5-Small performs only 0.31 and 0.15 points worse then the SLM (En-Fr and En-Ro), while T5-Large-2-T5-1.1-Small improves over T5-1.1-Small by around 3.4 points (En-Fr).
% Figure X puts these scores in relation to the inference runtime, showing that these benefits often come at a small runtime tradeoff compared to the SLM, and much faster than the LLM.
% We see these speedups already for 100 generated tokens (using also a prompt length of 100), which is close to the sequence lengths observed in WMT (mostly single sentences). More speedups can be expected for longer sequences due to the autoregressive nature of generation (see also Sect. 3.1) 

%TODO: add that we use add-concat for t5-3b to gpt2
%TODO: add that we use distillation for translation 

\begin{figure*}[htb]
  \centering
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{plots/pdf/LLM2SLM_translation_figure.pdf}
    % \caption*{Machine translation performance}
    \label{fig:1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=\textwidth]{plots/pdf/LLM2SLM_summarization_figure.pdf}
    % \caption*{Summarization performance}
    \label{fig:2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{plots/pdf/LLM2SLM_mtbench_figure.pdf}
    % \caption*{Instruction tuning performance}
    \label{fig:3}
  \end{subfigure}
  \vspace{-1\baselineskip}
  \caption{Performance-runtime comparison for various models across different tasks.}
  \label{fig:three-figures}
\end{figure*}


% \begin{figure}[t]
% \includegraphics[width=1.\linewidth]{plots/pdf/t5-perf-rt-llm2slm-fr-runtime.pdf}
% \caption{\textcolor{red}{Remove title so that table and figure toplines are aligned, increase model text font-size and potentially line-width, change color to blue (same as in tables), change model text according to tables. t5-large zero-shot text should go inside plot.}\textcolor{blue}{yuki: also add horizontal arrows that say "-500\%" runtime or something. } \textcolor{red}{For Amelie: Should be 3 columns (left: translation, center: summarization, right: instruction tuning) and contain averaged results which can be found in the respective column of each result table.}}
% \label{fig:runtime}
% %\vspace{-1em}
% \end{figure}

% WMT14 for En-Fr and En-De, train on train set, test on test set
% WMT16 for En-Ro, same setup
% T5 models, already pretrained for translation. Prefix: Translate ...
% T5-3B as LLM, and T5-Small and gpt2 as SLM
% train for 50k iterations


\subsection{Summarization}

We further assess the effect of combining models from different families for abstractive summarization on CNN/Daily Mail~\cite{hermann2015teaching}.
We again use T5 Large as LLM and connect a GPT2 as SLM.
%We do not employ T5-Small as an SLM, as the fine-tuned model exhibits only a narrow performance gap compared to the zero-shot evaluated T5-Large%~\cite{}.t5paper
Following~\citet{raffel2020exploring}, we prefix the prompt with "\texttt{summarize:}".
Similar to translation, T5 Large comes pretrained for summarization, so we skip the fine-tuning phase for it.
All other models are fine-tuned for 25k iterations on the training set and evaluated on the test split. 
In contrast to translation, ground truth labels are utilized because learning from them performs better than learning from LLM-generated labels.
ROUGE scores and runtimes are reported in \hyperref[tab:summarization]{Table~\ref{tab:summarization}}.
%We found, in contrast to translation, that using ground truth labels provided by the dataset works better than using distillation

\input{tables/summarization}
\input{tables/instruct}
GPT2 exhibits an average ROUGE score that is $1.24$ points lower than that of T5 Large.
In contrast, T5 Large$\,\to\,$GPT2 slightly exceeds the average score of T5 Large and shows a $3\times$ speedup, which is surprising since T5 Large is not trained in our \methodname{} and fine-tuning the SLM alone yields worse results. Importantly, our T5 Large$\,\to\,$GPT2 model performs on par with a fully fine-tuned GPT2 XL model while having a decoder which is $17\times$ smaller. %$3.8\times$ faster runtime and 
% We also fine-tune GPT2 XL and find that T5 Large$\,\to\,$GPT2 closely approaches its performance, but has a $17\times$ smaller decoder and is $3.8\times$ faster.

% fine-tuning GPT2, performance 1.x-1.5 points worse than LLM.
% T5-Large-2-GPT2 has better R-1 and R-LSum, which is surprising as we fix the LLM during fine-tuning, and SLM alone performs worse. Comparative performance in R2 and R-L.
%We also fine-tune a GPT2-XL on the task, and our LLM-2-SLM is very close in performance in particular for R-1 and R-L, despite being much smaller.

% CNN DailyMail (abstractive summarization)
% T5-3B and GPT2-XL as LLMs, gpt2 small as SLM
% T5-3B is pretrained on CNN DailyMail, we fine-tune GPT2-XL
% We do not use T5 small as SLM, as fine-tuning the model shows comparable results to T5-3b.
% prefix: summarize: 
% train models for 25k iterations
% rouge scores in table

%TODO: add that we use GT labels for summarization

%\subsection{Code generation}

% We now consider more challenging instruction tuning settings, in which networks are evaluated in a zero-shot manner on held-out tasks.
% Typically hard to evaluate, so we first consider code generation.
% Use the HumanEval benchmark, describe...
% describe eval metric
% use InstructCodeT5+ as LLM, and CodeT5+-Base/Large-Py, as well as CodeGen-Mono-Small as SLMs
% InstructCodeT5+ has been pretrained on... and CodeAlpaca
% We fine-tune all SLMs, as well as LLM-2-SLMs on CodeAlpaca
% We report pass rates in Table X.

%We now investigate the performance of our method in more challenging instruction tuning settings, in which models are evaluated in a zero-shot manner on held-out tasks.
%We use the HumanEval benchmark~\cite{chen2021evaluating}.
%We use InstructCodeT5+ as LLM, and CodeT5+-Base-Py, CodeT5+-Large-Py and CodeGen-Mono-Small as SLMs.
%We fine-tune all SLMs and LLM-2-SLMs on Code Alpaca~\cite{codealpaca}.



\subsection{Instruction tuning}

We explore the limits of our method in the %challenging
instruction tuning setting.
In contrast to traditional fine-tuning, where a single task is employed for training and evaluation, instruction-following models are trained for general problem solving on a multitude of tasks and evaluated on various held-out tasks.
We use Flan Alpaca XXL as LLM, which is a 11B parameter T5 trained on both Flan~\cite{chung2022scaling} - a collection of 1,800 tasks - as well as the Alpaca dataset~\cite{alpaca, wang2022self}, which consists of 52k generated instruction-following demonstrations.
%which consists of 52k instruction following demonstrations generated from OpenAI’s text-davinci-003.
For evaluation, we use the MT-bench dataset, which consists of 80 challenging tasks from 8 categories~\cite{zheng2023judging}.
As SLM, we utilize Flan T5 Base, i.e. a T5 that is only pretrained on Flan data, and fine-tune it on Alpaca data.
Note that our LLM, Flan Alpaca XXL, has $55\times$ more parameters than Flan T5 Base.
%As in~\cite{zheng2023judging}, we use GPT4 as a judge, their default prompt for single answer grading and the same sampling-based generation settings.

The results are reported in \hyperref[tab:instruct]{Table~\ref{tab:instruct}}.
Our LLM obtains an average score of $3.2$, and performs best in writing, extraction and roleplay.
In contrast, Flan Alpaca Base only has a relative score of $57.5\%$, which suggests that scale plays an important role.
We rerun this setting by fine-tuning Flan T5 Base on Alpaca data, and increase the score to $62.3\%$.
Our \methodname{} further increases the score to $73.4\%$, more than 10 percentage points better than the SLM alone and competing with a zero-shot evaluated Flan T5 XXL ($75.8\%$) and LLaMA 13B ($82.7\%$).
In addition, \hyperref[tab:instruct]{Table~\ref{tab:instruct}} indicates that our \methodname{} achieves a much better trade-off between performance and runtime compared to all other models.
Finally, we present qualitative examples in \hyperref[sec:appendix_mtbench]{Appendix~\ref{sec:appendix_mtbench}} %\hyperref[tab:instruct_examples]{Table~\ref{tab:instruct_examples}} in the Appendix 
demonstrating that our \methodname{} can produce fluent and sensible responses.

%We use the MT-bench dataset~\cite{zheng2023judging} for evaluation and use GPT4 as a judge~\cite{openai2023gpt4}.
%We fine-tune all SLMs and LLM-2-SLMs on the Alpaca dataset~\cite{alpaca}.
%We employ Flan-Alpaca-XXL and Llama-2-Chat as LLMs, and FLAN-T5-Base as SLM.

% We want to explore the limits of LLM-2-SLM in the more challenging instruction tuning setting.
%in contrast to traditional fine-tuning, where a single task is used for training and evaluation, in instruction tuning, a model is trained for general problem solving by training on multiple tasks and evaluating on various held-out tasks.
%We use T5 models that are already instruction tuned on Flan, which consists of over 1,800 tasks.
%Furthermore, we use models that subsequently were fine-tuned on the Alpaca dataset, which consists of 52k instruction following demonstrations generated from OpenAI’s text-davinci-003~\cite{alpaca, wang2022self}.
%For evaluation, we use the challenging MT-bench dataset consisting of 80 difficult tasks from 8 categories.
%We use the pretrained Flan-Alpaca-XXL as LLM and Flan-T5-Base as SLM.
%Flan-Alpaca-XXL has $55\times$ more parameters than Flan-T5-Base.
%As usual, we fix the LLM and train the SLM on Alpaca.
%For generation, we use the sampling strategy according to ...
%For evaluation, we use GPT4 as a judge as in ...
% As in Mt-bench paper, we use GPT4 as judge using their template for absolute scoring, as well as the same strategy for sampling across task categories.
%Scores are reported in table~\ref{tab:instruct}.
% LLM sucks in coding and math and performs best in writing, extraction and roleplay, which an average score of 3.15.
% Flan-Alpaca-Base (zero-shot) performs only 57.5% of LLM.
% Our own fine-tuned Flan-T5-Base on Alpaca dataset increases score to 62.3.
% Our LLM-2-SLM increases the score to 73.4%, more than 10 percentage points better than the SLM alone.
% We thus compete with a zero-shot evaluated Flan-T5-XXL (relative score: 75.8%) and a Llama-13B (82.7%).
%We note that we can only be as good as LLM.
% We show qualitative examples in Table 15, which demonstrates that LLM-2-SLM can produce fluent and senseful answers, which are considerably longer than in translation and summarization.
%Figure X shows runtimes, showing that 


%using the challenging MT-Bench dataset
%52K instruction-following demonstrations generated from OpenAI’s text-davinci-003 (alpaca + self-instruct citation)


\subsection{Runtime}

% Speedups between 2-4 times across tasks
% In translation, $4\times$ speedup, in summarization, 3\times (%$3.8\times$ faster runtime compared to GPT2XL), and in instruction tuning 2.32\times.
% Crucially, our \methodname{} is only marginally slower than the SLM, but performing significantly better.


\subsection{Ablation study}
\label{ss:ablation}
\paragraph{Tiny SLMs}
An alternative approach to improve inference efficiency is to downscale the SLM.
We revisit T5 Large$\,\to\,$GPT2 for machine translation and truncate the upper layers of a pretrained GPT2, resulting in GPT2 models with $L \in \{1, 2, 4\}$ layers, and only 8M, 15M, and 29M parameters, respectively.
\hyperref[fig:runtime_truncated_fr]{Figure~\ref{fig:runtime_truncated_fr}} demonstrates that \methodname{} models with truncated SLMs outperform corresponding SLM baselines by a wide margin while maintaining nearly the same runtime.
%\ya{random idea: just to beef up our results, can we show that we also get gains in the CPU-CPU case or GPU (LLM) - CPU (SLM) case?}

\begin{figure}[th]
\includegraphics[width=1.\linewidth]{plots/pdf/LLM2SLM_gpt2_figure.pdf}
\caption{Performance-runtime comparison with tiny GPT2 versions ($d$ indicates maximum depth) as SLMs for machine translation. The y-axis shows the average BLEU score across languages. 
T5 Large$\,\to\,$GPT2 with only 4 layers outperforms GPT2. The smaller the SLM, the greater the gap to our \methodname{} models.}
\label{fig:runtime_truncated_fr}
\end{figure}


\paragraph{Speculative decoding}
\label{ss:spec_dec}

%- in instruction tuning, llm2slm cannot quite compete with llm
%- but specdec to the rescue since it guarantees same performance as llm
%- problem with specdec is that llm runs multiple times
%- however, we show that we can still be X% faster then LLM
%- also, we are faster then specdec with the slm only

While our empirical evaluations on translation and summarization indicate that \methodname{} can achieve a comparable performance to the LLM, the instruction tuning results show that despite significant improvement over the SLM, \methodname{} may still lag behind the performance of the LLM.
This could be due to the evaluation regime (zero-shot on held-out tasks) and the breadth and complexity of the tasks in MT-bench.
Speculative sampling (SD), in contrast, guarantees matching the distribution of the LLM, even though the LLM has to be invoked multiple times~\cite{chen2023accelerating}.
%SD generates several tokens autoregressively with the SLM (draft model) and then uses the LLM (target model) to evaluate them.
%A subset of the SLM tokens is accepted and the next iteration begins.
Since our method is orthogonal to SD, we can apply it jointly to obtain LLM performance while still achieving substantial speedups.
%%we use the implementation of ... and report results in Table X.
Specifically, we consider our \methodname{}, Flan Alpaca XXL$\,\to\,$Flan T5 Base, as the draft model in which we apply the encoders of our LLM and SLM only once to encode the prompt.
We then repeatedly call the decoder of our SLM for autoregressive generation of the draft sequences.
The results reported in \hyperref[tab:sd_performance]{Table~\ref{tab:sd_performance}} show that we can match the performance of the LLM with our \methodname{}, while still being $1.8\times$ faster (compared to $2.3\times$ speedup of \methodname{} alone).
%Note that we are also more runtime efficient than the SLM with SD.
\input{tables/sd}


\paragraph{Parameter-efficient fine-tuning}

\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{lll}
\toprule
\textbf{Model} & \textbf{WMT} & \textbf{CNN/DN}\\
\midrule
Prompt tuning~\cite{lester2021power} & 25.06 & 19.52\\
Prefix tuning~\cite{li2021prefix} & 24.93 & 21.64\\
LoRA~\cite{hu2021lora} & 26.13 & 22.35\\
\midrule
\belowrulesepcolor{my-blue}
\rowcolor{my-blue}
\methodname{} (ours) & 30.27 & 24.13\\
\aboverulesepcolor{my-blue}
\bottomrule
\end{tabular}
}
\caption{PEFT results using fixed T5 Small for translation and GPT2 for summarization. Reported are average BLEU scores across languages (WMT) and average  ROUGE scores (CNN/DN). In our method, T5 Small and GPT2 are conditioned on T5 Large representations.}
\label{table:peft}
\end{table}

Our method has similarities with PEFT methods. In particular, soft prompt tuning prepends learnable tokens to the prompt embedding. In contrast, we add LLM representations element-wise to the prompt embedding of the SLM, which can be understood as a form of conditional prompting.
In \hyperref[table:peft]{Table \ref{table:peft}}, we compare the performance of PEFT methods with our approach by freezing the SLM and allowing only the training of the projector. Hyperparameters of the PEFT methods (see \hyperref[sec:peft_hyperparam]{Appendix~\ref{sec:peft_hyperparam}} for hyper-parameter details) are adjusted so that the total number of parameters matches our projector.
The results reported in \hyperref[table:peft]{Table \ref{table:peft}} show for both summarization and translation that our method outperforms all PEFT methods, indicating that conditioning on the LLM has a positive effect on performance compared to non-conditional approaches.

\paragraph{LLM vs. SLM tokenizer}

When using concatenation as fusion operator, the original tokenizer of the SLM may also be applied for \methodname{} variants that employ models of different families.
This also means that the down-projection and new header layers can be omitted.
In T5 Large$\,$GPT2, we found for translation that the LLM tokenizer performed better by 0.45 BLEU points (average across all languages), which could be due to the fact that the vocabulary of the T5 tokenizer also covers non-English languages.
%(30.38 vs. 30.83.)

\paragraph{Concatenation vs. addition}

\hyperref[tab:ablation_gt_gen]{Table~\ref{tab:ablation_gt_gen}} shows results for translation comparing concatenation and addition as fusion operator.
The results indicate that addition performs slightly better than concatenation.


\paragraph{Ground truth vs. LLM-generated labels}
In translation, we found that using labels generated by the LLM for training performs up to 1 BLEU point better than using ground truth labels (\hyperref[tab:ablation_gt_gen]{Table~\ref{tab:ablation_gt_gen}}). However, we point out that this is not generally the case. For summarization, the average rouge score is 0.44 points better when training with ground truth labels compared to LLM-generated labels.

\begin{table}[t]
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{lllll}
\toprule
\textbf{Model} & \makecell{\textbf{GT} \\ $+$} & \makecell{\textbf{GT} \\ \textbf{$\frown$}} & \makecell{\textbf{Gen.} \\ $+$} & \makecell{\textbf{Gen.} \\ $\frown$}\\
\midrule 
T5 Large$\,\to\,$T5 Small & 30.83 & \textcolor{orange}{30.63} & 31.54 & \textcolor{orange}{31.2} \\
T5 Large$\,\to\,$GPT2 & 29.68 & 29.71 & 31.05 & 30.83 \\
\bottomrule
\end{tabular}
}
\caption{Ablation of training signal and fusion operator, reporting average BLEU scores for translation across languages. GT: Ground truth labels, Gen.: Labels generated by T5 Large, $\frown$: Concatenation, $+$: Addition}
%\vspace{-1em}
\label{tab:ablation_gt_gen}
\end{table}



%\paragraph{General LLM}
%\textcolor{red}{Do we need a task fine-tuned LLM? Or are features coming from a generic pretrained model sufficient?
%Use mT5 and or T5 1.1. as LLM, train LLM-2-SLM on WMT at least.}

==> ethics.text/introduction.tex <==

The recent widespread adoption of large language models (LLMs)  enables a variety of applications in the field of natural language generation (NLG), from machine translation~\cite{wu2016google} and code completion~\cite{chen2021evaluating} to general-purpose chatbots that follow instructions~\cite{openai2023gpt4}.
%
Their performance is a function of compute, dataset size and parameter count~\cite{kaplan2020scaling, hoffmann2022training}, with emerging abilities becoming apparent only at large scale~\cite{thoppilan2022lamda, chowdhery2022palm, wei2022emergent}.
%These insights led to a rapid proliferation of model scaling, both in decoder-only architectures such as BLOOM~\cite{scao2022bloom}, OPT~\cite{zhang2022opt}, LLAMA-2~\cite{touvron2023llama}, and increasingly in encoder-decoder architectures such as FLAN-T5~\cite{chung2022scaling} and CodeT5+~\cite{wang2023codet5+}.
These insights have led to a rapid proliferation of model scaling, both in decoder-only~\cite{scao2022bloom, zhang2022opt, touvron2023llama} and increasingly in encoder-decoder networks~\cite{chung2022scaling, wang2023codet5p}.

As the race to scale intensifies, LLMs are becoming harder to operate, especially in light of compute limitations of edge devices and latency requirements, which ultimately translate into higher costs for providers and end users alike~\cite{chen2023frugalgpt}.
This is exacerbated by the way language models work, which in NLG problems can be characterized by two steps: (1) Encoding the task description and user prompt (e.g., \texttt{Translate into German: I love you}), which we summarize as prompt hereafter, followed by (2) decoding of the response (\texttt{Ich liebe dich}). %\footnote{Encoding is an overloaded term. Both encoder-decoder and decoder-only models are said to encode the prompt.}.
While the prompt for tasks such as translation or summarization is known in advance and can thus be processed efficiently in parallel, the response is usually generated in an autoregressive, sequential manner~\cite{radford2018improving, zarriess2021decoding}.
%\ya{it might make sense to give examples where all this is the case: fixed tasks: code completion, translation etc. need to steer reader away from classical language modelling}
Therefore, for each token to be generated, the LLM must be called, requiring all its weight matrices and the KV cache to be loaded.
As a result, decoding becomes bound to the memory bandwidth of the accelerator, which eventually leads to high inference latency as the length of the response grows~\cite{pope2023efficiently}.

\begin{figure}[tbp]
\includegraphics[width=.99\linewidth]{figures/llm2slm_fig1_bright.pdf}
\caption{\methodname: A large language model (LLM) computes a high-quality representation of the prompt to condition a small language model (SLM), which then efficiently decodes the response while maintaining high performance close to the LLM.}
\label{fig:llm2slm_highlevel}
\end{figure}

Research aimed at reducing the overall inference cost of LLMs has garnered significant interest over the past few years.
While traditional techniques, e.g. in model compression and conditional computation, are still active areas of research, recent developments show a pivot towards hybrid approaches.
For example, speculative decoding methods leverage a more efficient small language  model (SLM) to approximate the generation of an LLM~\cite{leviathan2023fast, chen2023accelerating}.
Others use cascades to run LLMs sequentially at varying costs~\cite{chen2023frugalgpt} or recycle LLM outputs for a small model~\cite{jiang2023recyclegpt}.
%that leverage a small language  model (SLM) approximating the generation of an LLM at a reduced inference cost via speculative decoding \cite{} or a cascade of LLMs with varying costs \cite{}. \ya{sentence too long, speculative decoding mentioned without proper intro/definition.} %despite the increased research focus on LLM efficiency via hybrid approaches~\cite{menghani2023efficient, treviso2023efficient},
Despite these promising developments, exploiting the discrepancy between fast prompt encoding and slow response generation remains under-explored. 

%This means that multiple calls to the LLM are required, and necessitates loading large weight matrices and KV cache (citation) for every to be generated token, which makes decoding memory bandwidth bound
%This means that each output token is computed sequentially, which necessitates multiple calls to the LLM and thus becomes slow and compute-expensive as the response grows in length.
%\ya{recommend to leave out this paragraph:} Despite the difference in efficiency, both steps are usually performed by either a single large network (decoder-only) or by sub-networks of similar size (encoder-decoder, such as Bart~\cite{lewis2019bart}, T5~\cite{raffel2020exploring}). 


%to enable more efficient language models remains underunexplored.

%LLM-2-SLM conditions an SLM with the prompt representation of an LLM, thus increasing the efficiency of autoregressive decoding while maintaining a high performance close to the LLM.

Intuitively, having a detailed understanding of the prompt is critical for the planning and delivery of an appropriate response.
In contrast, autoregressive decoding aims at predicting the next token, which is comparatively low-level and can in certain settings be accomplished well even by SLMs~\cite{eldan2023tinystories}.
%\methodname{} intends to leverage networks of different sizes for these complementary tasks.
To this end, we propose to reduce the cost of autoregressive decoding with a hybrid model in which these complementary tasks are distributed over two unequally sized networks (\hyperref[fig:llm2slm_highlevel]{Figure~\ref{fig:llm2slm_highlevel}}).
%Given that encoding the prompt can be done efficiently in parallel, computing LLM encoding to guide an SLM comes at a minor increase in overall computational costs for tasks requiring long sequence generation such as coding, summarization, instruction tuning, etc.
Specifically, we perform a single forward pass with an LLM to compute a high-quality representation of the prompt which is used to condition a more efficient SLM that then performs autoregressive generation.
Since the prompt can be encoded in parallel, computing an LLM representation to guide an SLM results in only a minor increase in overall computational cost compared to the SLM alone, in particular for tasks such as translation or instruction tuning that require generating longer sequences. We show that this minor increase in computational cost compared to the SLM allows for a substantial increase in performance.
Overall, we make the following contributions:
\begin{itemize}
    \item We present \methodname, a simple approach for fast autoregressive decoding where an LLM conditions an SLM. We mix LLM encoders with both encoder-decoder and decoder-only language models and only require fine-tuning of the SLM.
    \item We empirically study the performance and efficiency of different \methodname{} variants in various domains, training and evaluation regimes: traditional fine-tuning for both machine translation and summarization, as well as instruction-tuning evaluated in the zero-shot setting on multiple held-out tasks.
    \item Our method accelerates pretrained LLMs while maintaining high performance. For example, in translation, LLM-to-SLM achieves a $4.2\times$ speedup, with a marginal drop in performance of only $1\%$.
    
\end{itemize}


%Our method, called \methodname, can be used to accelerate pretrained LLMs $200-400\%$, often at a modest performance penalty.


%Furthermore, we only requires fine-tuning the attached SLM, which learns how to leverage the LLM encoding.
%By fine-tuning only the attached SLM to learn how to leverage the LLM encoding, we can mix both encoder-decoder and decoder-only language models as desired.

%\textcolor{red}{Overall, we make the following contributions}:
%\begin{itemize}
%    \item We propose \methodname{}, a novel framework for fast autoregressive decoding that uses a pretrained LLM for prompt encoding, and a fine-tuned SLM for generation.
%    We only require fine-tuning the SLM and can mix the LLM with both encoder-decoder and decoder-only SLMs.
%    \item We evaluate
%    \item Speed up autoregressive decoding compared to LLM alone by up to ..., converging towards runtime of the SLM.
%    showed efficacy on multiple benchmarks and showed that also possible for instruction tuning.
%    orthogonal to previous methods.
%\end{itemize}

%\ya{Intro is already a bit long, can you change this paragraph to a bullet-point list of "Overall we make the following contributions:" (list 3)}
%We empirically study the performance and efficiency of different \methodname{} variants in various domains, training and evaluation regimes: traditional fine-tuning for both machine translation on the WMT family of datasets and summarization on CNN / DailyMail, as well as instruction-tuning on Code Alpaca and Alpaca, evaluated in the zero-shot setting on multiple held-out tasks.
%We find that the difference in performance compared to the LLM alone is often marginal, even though the SLM is considerably smaller.
%\ya{too much detail for intro: }For example, we are able to mix a large InstructCodeT5+ model consisting of 16B parameters with a small 220M parameter CodeT5+ model fine-tuned on Code Alpaca, and observe a modest performance gap of \textcolor{red}{X points} on HumanEval compared to using the LLM only, while observing a \textcolor{red}{X} decoding speedup.
%We then ablate the impact of various design choices of our method on performance.
%Finally, we explore the limits of \methodname, by experimenting with even smaller models, down to \textcolor{red}{X} parameters, by truncating the upper layers of the SLM.
%Overall, our results suggest that hybrid models that transfer high-quality representations are a promising approach to reduce decoding costs while maintaining high performance, and may be of particular interest for latency-critical applications.
%\ya{intro definitely needs (ideally in the bullet point list) numbers like 500\% increase in speed at -0.1\% in performance or something. :)}
% experiments: We analyze the LLM-2-SLM framework on various domains, training and evaluation regimes and show that runtime compared to pure LLMs can be reduced considerably while maintaining competitive performance. We investigate the performance of LLM-2-SLM in the classic in-domain setting, where training and evaluation data come from the same distribution, as well as experiments on instruction-following training sets, where evaluation happens on out-of-domain datasets.
% ablation study: ablate design decisions of our method and experiment with even smaller SLMs by truncating the upper layers of the model further (larger gap in performance compared to the SLM-only setting).


%fine-tune and evaluate on translation to multiple language on WMT, summarization on CNN / DailyMail, code completion using CodeAlp and instruction tuning

%pretrained networks, fine-tune only SLM, low penalty in performance.

%Yet, encoding of the prompt and decoding of the response are usually either performed by the same network (decoder-only) or the respective networks are similar in size (encoder-decoder models). Although the trend towards ever larger models and autoregressive processing has led to an opposing research direction towards more efficient language models, exploiting the discrepancy between fast prompt encoding and slow response generation to enable more efficient language models is largely unexplored.

%(The trend towards increasing model sizes and autoregressive processing led to a contrasting line of research towards more efficient language models, including sparsity, pruning, speculative sampling, parallel decoding (citations)).


%

% we make use of the difference in efficiency between encoding and decoding and hypothesize that the representation quality of the prompt has large influence on generation quality.
%On that end, we  propose LLM-2-SLM, a hybrid approach
%where the prompt is encoded by an LLM, and the response is decoded by an SLM. is made considerably larger than the response decoder.
% thus, better representations
% use pretrained language models
% 

% experiments: We analyze the LLM-2-SLM framework on various domains, training and evaluation regimes and show that runtime compared to pure LLMs can be reduced considerably while maintaining competitive performance. We investigate the performance of LLM-2-SLM in the classic in-domain setting, where training and evaluation data come from the same distribution, as well as experiments on instruction-following training sets, where evaluation happens on out-of-domain datasets.


%fine-tune and evaluate on translation to multiple language on WMT, summarization on CNN / DailyMail, code completion using CodeAlp and instruction tuning




%LLMs for language generation operate in two phases: (1) encoding of a user prompt (e.g., Translate into German: I love you), (2) followed by decoding of the response (Ich liebe dich). The former,

%The working principle of LLMs is autoregressive decoding, where each to-be generated token requires one invocation of the model.

%


%The duality of model performance and cost has spurred a lot of research interest in LLM efficiency, e.g. pruning, sparsity, quantization, knowledge distillation...

==> ethics.text/limitations.tex <==
Although these results are promising, we have also identified limitations.
While the performance difference in traditional fine-tuning is often marginal, there is still a larger gap to the LLM in challenging settings such as instruction tuning.
In section~\ref{ss:spec_dec}, we demonstrate how this gap can be closed while still achieving a large increase in speed.
In addition, we only utilize encoder networks as LLMs at present. We provide preliminary results of decoder-only models as LLMs within our framework in \hyperref[sec:appendix_decoder_only]{Appendix \ref{sec:appendix_decoder_only}} and encourage the reader to continue exploring this promising direction.

==> ethics.text/method.tex <==

%Our method accelerates language generation by using networks of different sizes for prompt encoding and response decoding.
%Our method accelerates language generation by splitting it into parallel prompt encoding and autoregressive decoding and assigning networks of different sizes to these steps.
%Specifically, we utilize three modules: 

\begin{figure}[tbp]
\includegraphics[width=1.\linewidth]{figures/test3.pdf}
\caption{Architecture details. A frozen LLM integrates projected representations into either a trainable encoder-decoder or a decoder-only SLM.}

\label{fig:llm2slm_lowlevel}
\end{figure}


\iffalse Model capacity plays a crucial factor for LLM performance~\cite{kaplan2020scaling, hoffmann2022training}.
The main idea of \methodname{} is to address the low-capacity problem in SLM by introducing a high-quality LLM representation of the prompt which guides next token prediction in the SLM. % without incurring a large overhead in latency.
Intuitively, a detailed understanding of the prompt is critical for the planning and delivery of an appropriate response. %, which is technically motivated by the fact that computing each output token is a function of the prompt (Equation~\ref{eq:llm2slm}).
% THis also has technical motivation: each response token attends to all prompt encodings, as indicated by Equation 3.
%--- it is not without reason that each output token is a function of the prompt (Equation~\ref{eq:llm2slm}). %the representations of all prompt tokens .
On the other hand, autoregressive decoding aims at predicting the next token, which is comparatively low-level and can in certain settings be accomplished well even by SLMs~\cite{eldan2023tinystories}.
\methodname{} intends to leverage networks of different sizes for these complementary tasks.
%Even very small language models have been shown to produce grammatically correct sentences~\cite{eldan2023tinystories}.
Specifically, our method enables connecting an LLM encoder to both encoder-decoder and decoder-only SLMs, which can originate from the same or a different model family.
% Figure~\ref{fig:llm2slm_lowlevel} shows the components of \methodname{}, which are described in more detail next. 
\fi 








% \subsection{\methodname}

%We present \methodname, a method that combines language models to accelerate autoregressive decoding while maintaining high performance. 
It is well established that model capacity and overparametrization play a crucial factor in model performance~\cite{kaplan2020scaling, hoffmann2022training}.
Following this insight, the core idea of \methodname{} is to compensate the low parameter count of a small language model by conditioning its next token prediction on a high-quality representation of the prompt given by a LLM. 

\hyperref[fig:llm2slm_lowlevel]{Figure~\ref{fig:llm2slm_lowlevel}} presents an overview of \methodname:  First, the  \textbf{LLM} encoder $f_{\xi}$ computes a high-quality representation of the prompt.
The \textbf{projector} $q_{\phi}$ then adapts and projects this representation to the SLM embedding space.
Finally, the \textbf{SLM} $g_{\theta}$ takes the projected representation as input and generates the output tokens in an autoregressive manner.
%
Crucially, the parameter count of the SLM is significantly smaller than the LLM, leading to faster generation as only the SLM performs autoregressive decoding.
%Crucially, the modules are of different sizes, where parameter sets of LLM and SLM are related as follows: $|\xi|>|\theta|$. 
%\methodname{} allows for connecting an LLM encoder to both encoder-decoder and decoder-only SLMs, which can originate from the same or a different model family. 
% Figure~\ref{fig:llm2slm_highlevel} shows a high-level overview of our method. %, while Figure~\ref{fig:llm2slm_lowlevel} illustrates the architecture.
%and Figure~\ref{fig:llm2slm_lowlevel} illustrates the architecture.
In the rest of this section, we further describe each module of \methodname{}, and in particular how we inject the LLM's representations for both encoder-decoder and decoder-only SLMs.
%In the following, we first explain fast autoregressive decoding enabled by \methodname{} and then describe each module in more detail.%\textcolor{red}{We provide code at ....}.


% First formulate LLM-2-SLM as a means for fast autoregressive decoding, followed by describing several variants.

\subsection{Fast autoregressive decoding}

Given a prompt $X=\left[x_1,x_2,\dots,x_m\right]$ and an encoder-decoder LLM, 
autoregressive decoding models the output $Y=\left[y_1,y_2,...,y_n\right]$ in a causal manner:
%we are interested in a model $p(Y\vert X)$ that predicts the corresponding target sequence $Y=\left[y_1,y_2,...,y_n\right]$.
%When using an autoregressive model, each target token is computed sequentially from left to right in a causal manner.
%The distribution over output sequences can thus be written as a factorization of conditional distributions:
\begin{equation}
    p(Y\vert X)=\prod_{i=1}^{n} g_\xi(y_i\vert y_{<i}, f_\xi(x_{1:m}))
\end{equation}
where $f_\xi$ and $g_\xi$ refer to the LLM encoder and decoder respectively.
%
%
%where $\hat{y}_{<i}$ represents past inferred tokens.
%Commonly, each conditional is modeled by a single LLM:
%\begin{equation}
%    p(y_i|y_{<i},x_{1:m})=f_{\xi}(y_{<i}, x_{1:m}).
%\end{equation}
%
Generating the complete sequence $Y$ thus requires $n$ very costly forward  passes to the LLM decoder. 
%
Futhermore, these calls can not be parallelized as we need to first sample the token $y_i$ to estimate the probability distribution over the $i + 1$-th token.
%The generation of the complete sequence thus requires $n$ expensive calls of the LLM.
Instead, we propose to delegate the costly autoregressive decoding calls to a smaller language model, while preserving the encoder capacity:
\begin{equation}
    p(Y\vert X)=\prod_{i=1}^{n} g_{\theta}(y_{<i}, x_{1:m}, q_{\phi}( f_{\xi}(x_{1:m})))
    \label{eq:llm2slm}
\end{equation}
%\begin{equation}
%    p(y_i|y_{<i},x_{1:m})=g_{\theta}(y_{<i}, x_{1:m}, q_{\phi}( f_{\xi}(x_{1:m}))).
%    \label{eq:llm2slm}
%\end{equation}
The LLM is now only called once, to provide a high quality encoding of the input prompt  to the SLM.
%However, since each conditional distribution depends on the same prompt, we can compute $q_{\phi}( f_{\xi}(x_{1:m}))$ once and reuse it.
Therefore, as the number of autoregressive steps $M$ increases, the runtime of our method converges towards the original runtime of the SLM. %computational metrics such as FLOPs and runtime converge towards those of the SLM.

% In autoregressive sequence modeling, we are interested in predicting a target sequence Y=... given a prompt X=...

% In language generation problems, we are interested in generating the tokens of a target sequence Y=..., given a prompt X. = ..., we target to efficiently infer the target tokens Y = ... in an autoregressive manner.
% For training, one can use the cross-entropy loss, which can be factorized into conditional probabilities: ...
% which can be written as a product of conditional probabilities.
% Each probability term can be modeled as a function of a neural network, i.e. p(yi) = f_llm(X, y<i).
% We train this with the cross-entropy loss: ...
% in LLM-2-SLM, the probability instead can be modeled as a function of an SLM:
% Since LLM(x) in each term is  equivalent, we can rewrite
% 

% In language generation, given a prompt X={x1,x2,...,xn}, we are interested in predicting the corresponding target sequence Y={y1,y2,...,yn}.
% A common way to approach this is to use an autoregressive model where each token y_i is computed sequentially from left to right in a causal manner.

% A common way to approach this is to use an autoregressive model where each token y_i is calculated sequentially from left to right in a causal manner.

% We can train the parameters of such a model by minimizing the cross-entropy loss, which can be factorized into conditional probabilities of the respective target tokens: ...
% Commonly, each conditional is modelled by a single large language model f^{LLM}, i.e. (p(y_i|x = f_llm(x, y_<i).
% During training, the model can be efficiently trained in parallel using teacher forcing.
% However, during inference, generating the complete target sequence requires N calls of the LLM.
% Instead, we propose to increase efficiency of autoregressive generation by computing the conditional using a smaller model f^{SLM}: (p(y_i|x = f_slm(x, y_<i, f_llm(x)).
%Since the conditional does not vary with respect to x, one can precompute f_llm(x) once.

%We train this model using teacher forcing, and use both ground truth labels, as well as LLM-generated labels as target Y.


% \subsection{\methodname}

% It is well known that model capacity is a crucial factor for performance~\cite{kaplan2020scaling, hoffmann2022training}.
% The main idea of LLM-to-SLM is to address the low-capacity problem in smaller models by introducing a high-quality LLM representation of the prompt which guides next token prediction in the SLM. % without incurring a large overhead in latency.
% Intuitively, a detailed understanding of the prompt is critical for the planning and delivery of an appropriate response, which is technically motivated by the fact that computing each output token is a function of the prompt (Equation~\ref{eq:llm2slm}).
% % THis also has technical motivation: each response token attends to all prompt encodings, as indicated by Equation 3.
% %--- it is not without reason that each output token is a function of the prompt (Equation~\ref{eq:llm2slm}). %the representations of all prompt tokens .
% On the other hand, autoregressive decoding aims at predicting the next token, which is comparatively low-level and can in certain settings be accomplished well even by small language models~\cite{eldan2023tinystories}.
% \methodname{} intends to leverage networks of different sizes for these complementary tasks.
% %Even very small language models have been shown to produce grammatically correct sentences~\cite{eldan2023tinystories}.
% Specifically, our method enables connecting an LLM encoder to both encoder-decoder and decoder-only SLMs, which can originate from the same or a different model family.
% Figure~\ref{fig:llm2slm_lowlevel} shows the components of \methodname{}, which are described in more detail next. 



%Specifically, we interconnect an LLM encoder with an encoder-decoder or decoder-only SLM to enable more efficient decoding.
%\textcolor{red}{Since two networks are involved, there is an inherent similarity to the original transformer~\cite{vaswani2017attention}.
%We follow the same high-level structure, where the LLM can be considered as an encoder and the SLM as a decoder.}

% The main idea of LLM-to-SLM, is to resolve the missing capacity problem by introducing a high-quality LLM representation of a prompt, in order to better guide next-token predicton. 
% Conceptually, a proper understanding of the prompt is critical to generate an appropriate answer.
%The response is dependent on the prompt,.
%Technically, as shown in Eq. 3, each output token to be generated, attends to this representation.
% and  and we hypothesize that a better representation of it will likely leed to better performance.


%We leverage pretrained language models and fine-tune the SLM using teacher forcing. Thus, as indicated in Eq.X, the target sequence is used as additional input to predict the respective next token, in a single parallel forward pass.
%In the following, we describe the different modules and variants of our method in more detail.

\subsection{Architecture}
%\subsubsection{LLM encoder}
\paragraph{LLM encoder.}
%The LLM encoder $f_{\xi}:X\mapsto H$ takes a prompt $X$ of length $m$ as input and computes a high-quality representation $H\in\mathbb{R}^{m\times d_l}$ of it.
%For this purpose, the prompt is first embedded and then passed to a standard transformer encoder~\cite{vaswani2017attention}, which consists of multiple blocks of bi-directional multi-head self-attention, multilayer perceptron (MLP), residual connections and Layernorms.

In training LLMs, the requirement for substantial computational resources is often a limiting factor.
%Typically, a substantial accelerator budget is required for training LLMs.
In our approach, we focus on a more resource-efficient training regime closer to that of the SLM, by freezing the parameters of the LLM during fine-tuning.
In this way, we can train \methodname{} on a small budget by pre-computing prompt representations.
To ensure good representation quality, we leverage large pretrained encoder-decoder models, but omit the decoder. The last layer representation of the encoder in an encoder-decoder architecture serves as a straightforward prompt encoding point for an SLM. In a decoder only model, in contrast, determining the exact intermediate layer(s) that contribute to encoding of the prompt is more challenging as the last layer representation is mainly useful for the low-level task of predicting the next token~\cite{chen2020generative}. In \hyperref[sec:appendix_decoder_only]{Appendix \ref{sec:appendix_decoder_only}} we present preliminary results for using a decoder only LLM in our \methodname{} framework.

\iffalse This ensures that we can always use the last layer representation that was already being used by the previously connected pretrained decoder.
In contrast, decoder-only models may learn useful features only in an intermediate layer, where the last layer representation is mainly useful for the low-level task of predicting the next token~\cite{chen2020generative}. \fi


% We use the final representation of the encoder
%We made this design choice opposed to decoder-only models, since encoder representations have previously been trained to be transferred to a decoder, as opposed to decoder-only models, where the last layer representation is concerned with next token prediction.

%of multiple bi-directional transformer block

%For this purpose, the prompt is first embedded and, depending on the model, a position encoding may be added.
%Then, in line with the standard transformer encoder~\cite{vaswani2017attention}, a series of transformer blocks is executed.
%Since the prompt is known in advance, we utilize bi-directional attention so that each token can attend to itself and every other token.
%Each block thus consists of multi-head self-attention (MHSA), followed by a multilayer perceptron (MLP).
%Residual connections are applied both after MHSA and MLP, and a Layernorm is placed either before or after each of these layers, depending on the choice of language model~\cite{wang2019learning}.
%Depending on the specific choice of the LLM, residual connections and Layernorm, following the encoder of a standard transformer~\cite{vaswani2017attention}.
%\ya{this is implementation detail, consider moving to another section. Rather talk about the non-trivial problems that arise and that necessitate our method? different dimensions/ non-aligned representation spaces, different tokenizers. these might better guide your method section too, otherwise everything seems too trivial.}

%For the experiments, we use pretrained T5 encoder-decoder models as LLMs (see Table~\ref{table:models}), but omit the decoder.
%Furthermore, we freeze the parameters of the LLM during fine-tuning.
%It is thus possible to train with our method on a small accelerator budget by computing prompt representations in advance.

\paragraph{Projector.}
The projector $q_{\phi}:H\mapsto Z$ has the task of aligning representations between LLM and SLM.
It takes high-dimensional features $H\in\mathbb{R}^{m\times d_l}$ of the LLM as input and computes a lower-dimensional representation $Z\in\mathbb{R}^{m\times d_s}$ which can be fused directly with embeddings of the SLM. %embeddings and/or intermediate 
Although there are many ways to design such a projector, we found that using a small MLP: \texttt{Linear($d_l$, $d_s$)} $\to$ \texttt{ReLU} $\to$ \texttt{Linear($d_s$, $d_s$)} trained from scratch is simple, efficient and performs well.



\paragraph{SLM.}
The SLM $g_{\theta}:(X,Z)\mapsto\hat{Y}$ maps the tokenized input $X$ and the projected representation $Z\in\mathbb{R}^{m\times d_s}$ to the response $\hat{Y}$ of length $n$.
During training, we further append the target sequence $Y$ to the input to enable next token prediction via teacher forcing~\cite{williams1989learning}.
Equivalently, previously predicted tokens $\hat{y}_{<i}$ are appended during inference.
We employ pretrained networks as SLMs, but fine-tune them as they have not been previously trained to process high-capacity encodings.

To integrate the projected LLM representation into the SLM, the tokenized input ($X|Y \text{or }  \hat{y}_{<i}$) is first embedded.
A straightforward way to fuse features is to replace the SLM embedding with the projected LLM representation.
This is similar to soft prompt tuning~\cite{lester2021power}, with the difference that our prompts are conditional.
However, we found empirically that adding the projected LLM representation onto the SLM embedding performs better (see also Section~\ref{ss:ablation}).
In this way, we preserve the semantics between the SLM embeddings of prompt and target/predicted sequence and leverage the LLM representation to modulate the prompt embedding via addition.
Note that there are various other options for fusing the features of different models, e.g. cross-attention, or FiLM layers~\cite{perez2018film}. However, We opted for adding, as it is simple and requires minimal changes to the SLM.
The fused joint representation is finally fed into the SLM, which is either an encoder-decoder or a decoder-only transformer model.

%We first embed the tokenized input and then fuse it with the LLM features.
% A simple way of feature fusion is to replace the prompt embeddings computed by the SLM with the LLM representation.

%

%To condition the SLM, we first embed the tokenized input and then add the projected LLM representation.
%Empirically, we found this to work better than inserting the LLM representation directly into the SLM (see also Section~\ref{ss:ablation}).
%After tokenization, the input is first embedded and subsequently added to the projected LLM representation.


%Note that concatenating features

%In more detail, the input is first embedded. Then, the projected representation is added. The fused representation is then input to either an encoder-decoder or decoder-only SLM.
\subsection{SLM architecture variants}
\subsubsection{Encoder-decoder}
% Adding the projected LLM representation and embedding requires aligned sequence lengths of LLM representation and prompt embedding. 

%Since the SLM shares the same tokenizer as the LLM, we can embed the input directly with the embedding matrix of the SLM.
Similar to the LLM, the SLM encoder also applies multiple bi-directional attention blocks.
%Similar to the LLM, multiple bi-directional attention blocks are executed.
The SLM decoder then takes a start-of-sequence token, as well as the target sequence (or previously predicted tokens during inference) as input and executes alternating blocks of cross-attention and causal self-attention.
%Crucially, each cross-attention layer attends to the output of the SLM encoder, denoted as $Z^*$, which in turn is a function of the LLM representation:
Each cross-attention layer attends to the output of the SLM encoder, which in turn is a function of $Z$.
%The output of the SLM encoder is then forwarded to the decoder, which consists of 
%For decoding, each cross-attention layer attends to the representation of the SLM encoder, denoted as $Z^*$, which in turn is a function of the projected LLM representation:
%followed by a linear head.
%For this purpose, the input is first tokenized, and subsequently embedded.
%Then, the projected representation Z is added to the embedding.
%The SLM then
%We employ various smaller-sized pretrained T5s as cross-attention based SLMs.
%Contrary to the large model, we apply only the decoder and omit the encoder.
%The structure of the SLM depends on its model type, as well as the tokenizer of the LLM.
%For encoder-decoder SLMs, we omit the encoder and provide a start-of-sequence token (SoS) as input to the decoder.
%Since the SLM shares the same tokenizer as the LLM, we can embed the input directly with the embedding matrix of the SLM.
%In line with the standard transformer decoder~\cite{vaswani2017attention}, a series of $\ell_{S}$ consecutive cross-attention and causal attention blocks\footnote{Both transformer blocks adopt the same general structure as the bi-directional block, only with different inputs or attention masks.} are employed, followed by a linear head.
%Crucially, the cross-attention layer integrates the projected LLM representation into the SLM:
%\begin{subequations}
%\begin{align}
%    Q &= AW_q, \quad \texttt{ \textcolor{my-green}{\# queries}} \\
%    K &= Z^*W_k, \quad \texttt{\textcolor{my-green}{\# keys}}\\
%    V &= Z^*W_v, \quad \texttt{\textcolor{my-green}{\# values}}\\
%    \mathrm{Att.}(Q,K,V) &= \mathrm{Softmax}\left(\frac{Q K^T}{\sqrt{d_S}}\right),
%\end{align}
%\end{subequations}
%where $A\in\mathbb{R}^{n\times d_s}$ is an intermediate SLM representation (layer indices omitted for brevity), and $W_q, W_k\in\mathbb{R}^{d_s\times d_k}$, $W_V\in\mathbb{R}^{d_s\times d_k}$ and $d_k$, $d_v$ being the key and value dimensions, respectively.
After the final block, a linear head is applied, which maps to the output vocabulary.
In the experiments, we utilize multiple smaller-sized pretrained encoder-decoder SLMs and fine-tune them.

\subsubsection{Decoder-only}

In order to fuse the LLM representation with the input embedding via addition, sequence lengths must be aligned.
This is naturally the case for models of the same family that use the same tokenizer and vocabulary.
However, when connecting decoder-only SLMs to LLM encoder models, the vocabularies may not match in practice, resulting in sequences of different lengths.
Therefore, we propose to reuse the tokenizer and the embedding matrix of the LLM to align sequence lengths.
We further apply a linear down-projection layer to adjust the embedding dimension from $d_l$ to $d_s$.
The joint embedding is then passed to the decoder-only SLM, which consists of multiple blocks that use the causal self-attention mechanism, where each token attends to both itself and the past.
Finally, a new linear head is employed that maps to the vocabulary of the LLM tokenizer.
%We use pretrained GPT2 models as decoder-only SLMs and fine-tune them.

%When using models of the same family, e.g. when using T5s for both LLM and SLM, the tokenizer and vocabulary is the same

%Decoder-only models only adopt the causal self-attention mechanism, where each token attends to both itself and the past.



%To integrate the LLM representation with minimal changes into the SLM, we explore two approaches.
%The first involves inserting the LLM representation directly into the SLM via embedding concatenation, where $X_{dec}$ remains empty.
%During training, given left-padded token embeddings of the target sequence $E_Y^{pad}\in\mathbb{R}^{(m+n)\times d_S}$, where $E_Y^{pad}[0:m]=0$, and right-padded projected LLM representations $Z^{pad}$ of same dimension, where $Z^{pad}[m:m+n]=0$, we concatenate them to obtain the initial SLM representation $A^0$:
%\begin{equation}
%    A^0 = Z^{pad} + E_Y^{pad}.
%\end{equation}
%
%The second approach, which performs better empirically and is used in the main experiments, sets $X_{dec}=X$ and thus add-concatenates the joint embedding $E_{X\,|\,Y}$ of prompt and target sequence with the LLM representation:
%\begin{equation}
%    A^0 = Z^{pad} + E_{X\,|\,Y}.
%    \label{eq:add_concat}
%\end{equation}
%In other words, we preserve semantics between input prompt and target sequence, and utilize the LLM representation to modulate the prompt embedding via addition.
%Equation~\ref{eq:add_concat} requires aligning sequence lengths of LLM representation and prompt embedding. 
%In practice, this is not guaranteed as different model families use different tokenizer vocabularies.
%Therefore, we propose to reuse the tokenizer and embedding matrix of the LLM to embed both prompt and target sequence, followed by a down-projection onto the dimension of the SLM using a single linear layer.
%Finally, a new linear head maps to the vocabulary of the LLM tokenizer.

%The second approach leverages the existing SLM representations of the input prompt, by adding the corresponding embeddings to the LLM representation.

%We found that a slightly better performing alternative is to add the LLM representation to the embeddings of the input prompt, before concatenating them the the target token embeddings.
% because we can preserve the features the SLM network is used to.
% has similarities to prompt learning
%The latter approach requires that the sequence lengths of LLM representation and SLM embedding match, which requires the use of the same tokenizer.
%Therefore, we employ the LLM tokenizer and embedding matrix, followed by down-projection. We also employ a new linear head that maps to the vocabulary of the LLM.

%\paragraph{SLM} The structure of the SLM depends on both the employed tokenizer, as well as on whether an encoder-decoder or decoder-only model is used. For encoder-decoder SLMs, such as T5-Small, an start-of-sequence token (SoS) is used. During training, the target sequence is prepended, in order to learn via teacher forcing (citation).
% The embedding matrix to be used depends on whether the tokenizer of the SLM if the same used for the LLM. For models within the same family (e.g. T5-Large-2-T5-Small), we can simply use the embedding matrix of the SLM.
% However, if a different tokenizer is used (e.g., T5-Large-2-GPT2), 

% The SLM takes the projected representation and, during training, the target sequence as input and outputs a corresponding response using teacher forcing (citation). The structure of the SLM and in particular the way in which the LLM representation is processed depends on the model type.
% For encoder-decoder SLMs, such as T5-Small, a start-of-sequence (SoS) token is prepended to the target sequence. The corresponding features then form the queries, and keys and values are computed based on the LLM representation:

%we can compute cross-attention, using the ...: formula.
% This is followed by a causal-attention transformer block, where each token attends to itself and the past, only.
% For decoder-only SLMs (such as GPT2), we can concatenate the projected LLM representation

%\paragraph{LLM}
% The LLM takes an input prompt and computes a high-quality representation of it.
% First, the input prompt is tokenized and embedded by the tokenizer and embedding matrix of the LLM.
% Then, $L_{LLM}$ transformer blocks are executed. Each block consists of Multi-head Self-Attention, an MLP, residual connections and Layernorms, following the encoder of the standard transformer (Vaswani paper citation).
% The output of the LLM is a representation of the input prompt.
% Note that the LLM is frozen. We can thus store the representations on disk, so that we can train LLM-2-SLM on consumer-scale GPUs.
% Note that we use bi-directional attention, as is used in encoder-decoder architectures. We also tried decoder-only LLMs, but found them to not work well. One reason for this might be that the last layer representations are useful for predicting the next token, which might not be a good representation for the semantics of the prompt.

%\paragraph{Projector} The projector ...: h --> z maps the representation computed by the LLM to an aligned representation z, that can be used directly by the SLM. We use a small MLP (Linear(D, d), ReLU, Linear(d,d) and train it from scratch.

%\subsubsection{Training details}

% Used models are shown in Table X.
% For translation and summarization, we use T5-Large as LLM and T5-Small, T5-1.1-Small and GPT2 as SLMs

% Train either on GT or distillation.




%\paragraph{Encoder-Decoder-2-Encoder-Decoder}

%\paragraph{Encoder-Decoder-2-Decoder-Only}

%\paragraph{Decoder-only-2-Decoder-only}

==> sections/discussions.tex <==
...
%  hypothesized that higher importance can be ascribed to the quality of the prompt representation. not least because it guides response generation and narrows down the set of sensible responses. also, every decoding step attends to prompt
% decoder instead has the more low-level task of producing only the next token, which should be simpler than understanding the semantics of the prompt.
% can be seen in the results that this holds true...

==> tables/all_raw_tables.tex <==

\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{lcc}
\hline
\textbf{Model} & \textbf{Dataset} & \textbf{Performance}\\
\hline
t5-small & WMT14 en-fr & 35.54 \\
t5-base & WMT14 en-fr & 38.27\\
t5-large & WMT14 en-fr & 39.53\\ 
t5-3b & WMT14 en-fr & 39.57 \\ 
t5-small & WMT14 en-de & 24.98\\
t5-base & WMT14 en-de & 27.82\\ 
t5-large & WMT14 en-de & 29.10\\ 
t5-3b & WMT14 en-de & 29.11\\
t5-small & WMT16 en-ro & 25.53\\
t5-base & WMT16 en-ro & 26.54\\ 
t5-large & WMT16 en-ro & 27.19\\ 
t5-3b & WMT16 en-ro & 27.28\\
t5-small & CNN & 36.89, 16.67, 26.61, 34.23\\
t5-base & CNN & 38.73, 17.87, 27.72, 35.94\\ 
t5-large & CNN & 40.07, 18.84, 28.82, 37.30\\ 
t5-3b & CNN & 41.33, 19.93, 29.83, 38.44\\\hline
\end{tabular}
}
\caption{Test set zero-shot performances. BLEU for translation (single metric) or ROUGE (ROUGE-1, ROUGE-2, ROUGE-L, ROUGE-LSUM).}
\label{tab:accents}
\end{table}

\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{llll}
\hline
\textbf{Model} & \textbf{Feature fusion} & \textbf{Target source} & \textbf{BLEU 5, 50k}\\
\hline
t5-small & - & GT & 32.25, 36.48 \\
t5-small & - & T5-large-gen & 36.41, 37.16 \\
t5-1.1-small & - & GT & 15.16, 32.06 \\
t5-1.1-small & - & T5-large-gen & 19.83, 34.85 \\
T5-large-2-t5-small & Concat & GT & -, 37.44 \\
T5-large-2-t5-small & Add-Concat & GT & -, 38.14 \\
T5-large-2-t5-small & Concat & T5-large-gen & 35.86, 38.95 \\
T5-large-2-t5-small & Add-Concat & T5-large-gen & 37.5, 39.22 \\
T5-3b-2-t5-small & Add-Concat & T5-3b-gen & 37.43, 38.68, 39.31 (100k) \\
T5-large-2-t5-1.1-small & Concat & GT & -, 35.54 \\
T5-large-2-t5-1.1-small & Add-Concat & GT & -, 35.42 \\
T5-large-2-t5-1.1-small & Concat & T5-large-gen & 27.5, 38.08 \\
T5-large-2-t5-1.1-small & Add-Concat & T5-large-gen & -, 38.21 \\
gpt2 & - & GT & 25.17, 33.36 \\
gpt2 & - & T5-large-gen & 30.23, 35.67 \\
gpt2 w T5 tokenizer & - & GT & 17.70, 30.33 \\
gpt2 w T5 tokenizer & - & T5-large-gen & 23.20, 33.53 \\
T5-large-2-gpt2 & Concat & GT & 24.35, 37.54 \\
T5-large-2-gpt2 & Add-Concat & GT & 24.44, 37.26 \\
T5-large-2-gpt2 & Concat & T5-large-gen & 30.32, 39.00 \\
T5-large-2-gpt2 & Add-Concat & T5-large-gen & 30.75, 39.01 \\\hline
\end{tabular}
}
\caption{BLEU scores on WMT14 English to French}
\label{tab:accents}
\end{table}

\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{llll}
\hline
\textbf{Model} & \textbf{Feature fusion} & \textbf{Target source} & \textbf{BLEU 50k}\\
\hline
t5-small & - & GT & 26.11 \\
t5-small & - & T5-large-gen & 26.15 \\
t5-1.1-small & - & GT & 24.83 \\
t5-1.1-small & - & T5-large-gen & 25.25 \\
T5-large-2-t5-small & Concat & GT & 26.36 \\
T5-large-2-t5-small & Add-Concat & GT & 27.06 \\
T5-large-2-t5-small & Concat & T5-large-gen & 26.59 \\
T5-large-2-t5-small & Add-Concat & T5-large-gen & 27.04 \\
T5-large-2-t5-1.1-small & Concat & GT & 25.37 \\
T5-large-2-t5-1.1-small & Add-Concat & GT & 26.05 \\
T5-large-2-t5-1.1-small & Concat & T5-large-gen & 25.93 \\
T5-large-2-t5-1.1-small & Add-Concat & T5-large-gen & 26.54 \\
gpt2 & - & GT & 23.78 \\
gpt2 & - & T5-large-gen & 24.70 \\
T5-large-2-gpt2 & Concat & GT & 24.67 \\
T5-large-2-gpt2 & Add-Concat & GT & 24.95 \\
T5-large-2-gpt2 & Concat & T5-large-gen & 25.38 \\
T5-large-2-gpt2 & Add-Concat & T5-large-gen & 25.86 \\\hline
\end{tabular}
}
\caption{BLEU scores on WMT16 English to Romanian}
\label{tab:accents}
\end{table}

\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{llll}
\hline
\textbf{Model} & \textbf{Feature fusion} & \textbf{Target source} & \textbf{BLEU 50k}\\
\hline
t5-small & - & GT & 25.46 \\
t5-small & - & T5-large-gen & 26.47 \\
t5-1.1-small & - & GT & 22.13 \\
t5-1.1-small & - & T5-large-gen & 24.55 \\
T5-large-2-t5-small & Concat & GT & 26.83 \\
T5-large-2-t5-small & Add-Concat & GT & 27.28 \\
T5-large-2-t5-small & Concat & T5-large-gen & 28.04 \\
T5-large-2-t5-small & Add-Concat & T5-large-gen & 28.36 \\
T5-large-2-t5-1.1-small & Concat & GT & 25.48 \\
T5-large-2-t5-1.1-small & Add-Concat & GT & 25.47 \\
T5-large-2-t5-1.1-small & Concat & T5-large-gen & 27.40 \\
T5-large-2-t5-1.1-small & Add-Concat & T5-large-gen & 27.42 \\
gpt2 & - & GT & 23.70 \\
gpt2 & - & T5-large-gen & 25.53 \\
T5-large-2-gpt2 & Concat & GT & See TODO \\ %TODO: /prj/corp/crd/morpheus/lasvegas/model_efficiency/bbergner/experiments/kangaroo/t5distill/wmt-de-t5-gt-gpt2-1tokenizer_lr=0.001_num-iterations=50000_model-arch=gpt2_tokenizer-name=t5-small_tokenizer-slm-name=t5-small_hard-prompt=eleventh/log.out
T5-large-2-gpt2 & Add-Concat & GT & See TODO  \\ %TODO: /prj/corp/crd/morpheus/lasvegas/model_efficiency/bbergner/experiments/kangaroo/t5distill/wmt-de-t5-gt-add-gpt2-1tokenizer_lr=0.001_num-iterations=50000_model-arch=gpt2_tokenizer-name=t5-small_tokenizer-slm-name=t5-small_hard-prompt=eleventh/log.out
T5-large-2-gpt2 & Concat & T5-large-gen & 28.13 \\
T5-large-2-gpt2 & Add-Concat & T5-large-gen & 28.27 \\\hline
\end{tabular}
}
\caption{BLEU scores on WMT14 English to German}
\label{tab:accents}
\end{table}

\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{llll}
\hline
\textbf{Model} & \textbf{Feature fusion} & \textbf{Target source} & \textbf{ROUGE (up to 50k)}\\
\hline
gpt2 & - & GT & 38.58, 17.56, 27.36, 36.06 \\
gpt2 & - & T5-large-gen & 37.75, 17.06, 26.94, 35.18 \\
gpt2 w T5 tokenizer & - & GT & 36.76, 16.05, 25.83, 34.01 (40k) \\
gpt2 w T5 tokenizer & - & T5-large-gen & 36.66, 16.08, 25.93, 33.83 (40k) \\
T5-large-2-gpt2 & Concat & GT & 40.22, 18.64, 28.80, 37.64 (25k) \\
T5-large-2-gpt2 & Add-Concat & GT & 40.04, 18.36, 28.52, 37.42 (25k) \\
T5-large-2-gpt2 & Concat & T5-large-gen & 39.47, 18.36, 28.50, 36.79 (25k) \\
T5-large-2-gpt2 & Add-Concat & T5-large-gen & 39.13, 18.15, 28.27, 36.48 (25k) \\
gpt2-xl-2-gpt2 & Add-Concat & GT & - \\
gpt2-xl-2-gpt2 & Add-Concat & gpt2-xl-gen & - \\
gpt2-xl-2-gpt2 & Concat & gpt2-xl-gen & - \\\hline
\end{tabular}
}
\caption{ROUGE scores (1, 2, L, SUM) on CNN}
\label{tab:accents}
\end{table}


\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{llll}
\hline
\textbf{Model} & Dataset & \textbf{\#SLM layers} & \textbf{BLEU 50k}\\
\hline
gpt2 & WMT14 En-Fr & 1 & 13.15 \\
gpt2 & WMT14 En-Fr & 2 & 29.34 \\
gpt2 & WMT14 En-Fr & 4 & 32.39 \\
gpt2 & WMT14 En-Fr & 12 & 35.67\\
T5-large-2-gpt2 & WMT14 En-Fr & 1 & 25.00 \\
T5-large-2-gpt2 & WMT14 En-Fr & 2 & 35.37 \\
T5-large-2-gpt2 & WMT14 En-Fr & 4 & 37.98 \\
T5-large-2-gpt2 & WMT14 En-Fr & 12 & 39.01 \\
gpt2 & WMT14 En-De & 1 & 6.59 \\
gpt2 & WMT14 En-De & 2 & 19.43 \\
gpt2 & WMT14 En-De & 4 & 22.57 \\
gpt2 & WMT14 En-De & 12 & 25.53 \\
T5-large-2-gpt2 & WMT14 En-De & 1 & 17.16 \\
T5-large-2-gpt2 & WMT14 En-De & 2 & 25.07 \\
T5-large-2-gpt2 & WMT14 En-De & 4 & 27.36 \\ %TODO: /prj/corp/crd/morpheus/lasvegas/model_efficiency/bbergner/experiments/kangaroo/t5distill/wmt-de-t5-distill-add-gpt2-4-layers-2nd-1tokenizer_lr=0.001_num-iterations=50000_model-arch=gpt2_tokenizer-name=t5-small_tokenizer-slm-name=t5-small_hard-prompt=eleventh/log.out
T5-large-2-gpt2 & WMT14 En-De & 12 & 28.27 \\
gpt2 & WMT14 En-Ro & 1 & 8.65 \\
gpt2 & WMT14 En-Ro & 2 & 20.39 \\
gpt2 & WMT14 En-Ro & 4 & 22.61 \\
gpt2 & WMT14 En-Ro & 12 & 24.70 \\
T5-large-2-gpt2 & WMT14 En-Ro & 1 & 17.39 \\
T5-large-2-gpt2 & WMT14 En-Ro & 2 & 23.79 \\
T5-large-2-gpt2 & WMT14 En-Ro & 4 & 25.25 \\
T5-large-2-gpt2 & WMT14 En-Ro & 12 & 25.86\\
\hline
gpt2 & avg & 1 & 9.46 \\
gpt2 & avg & 2 & 23.05 \\
gpt2 & avg & 4 & 25.86 \\
gpt2 & avg & 12 & 28.63 \\
T5-large-2-gpt2 & avg & 1 & 19.85 \\
T5-large-2-gpt2 & avg & 2 & 28.08 \\
T5-large-2-gpt2 & avg & 4 & 30.20 \\
T5-large-2-gpt2 & avg & 12 & 31.05 \\
\\\hline
\end{tabular}
}
\caption{Layer trunction ablation, using distillation targets, and Add-Concat fusion in LLM-2-SLM}
\label{tab:accents}
\end{table}

\begin{table}
\centering
\noindent\adjustbox{max width=\linewidth}{
\begin{tabular}{lllll}
\hline
\textbf{Model} & \textbf{\#Tokens} & \textbf{\#Params} & \textbf{GFLOPs} & \textbf{Runtime [s]}\\
\hline
T5-small & 100 & 60.51 & 12.41 & 1.42 \\
T5-small & 500 & 60.51 & 45.17 & 7.18 \\
T5-base & 100 & 222.90 & 45.51 & 2.94 \\
T5-base & 500 & 222.90 & 150.46 & 15.17 \\
T5-large & 100 & 737.67 & 150.00 & 6.15 \\
T5-large & 500 & 737.67 & 474.03 & 29.91 \\
gpt2-small & 100 & 124.44 & 50.11 & 1.97 \\
gpt2-small & 500 & 124.44 & 154.92 & 9.83 \\
gpt2-4-layers & 100 & 67.74 & 26.59 & 0.74 \\
gpt2-4-layers & 500 & 67.74 & 82.47 & 3.50 \\
gpt2-2-layers & 100 & 53.56 & 21.15 & 0.39 \\
gpt2-2-layers & 500 & 53.56 & 64.36 & 1.98 \\
gpt2-1-layer & 100 & 46.47 & 18.26 & 0.24 \\
gpt2-1-layer & 500 & 46.47 & 55.3 & 1.19 \\
T5-large-2-T5-small & 100 & 789.96 & 73.96 & 1.48 \\
T5-large-2-T5-small & 500 & 789.96 & 106.72 & 7.52 \\
T5-large-2-gpt2-small & 100 & 883.25 & 106.87 & 2.07 \\
T5-large-2-gpt2-small & 500 & 883.25 & 201.80 & 9.77 \\
T5-large-2-gpt2-4-layers & 100 & 826.25 & 83.70 & 0.75 \\
T5-large-2-gpt2-4-layers & 500 & 826.25 & 129.34 & 3.69 \\
T5-large-2-gpt2-2-layers & 100 & 812.37 & 77.91 & 0.43 \\
T5-large-2-gpt2-2-layers & 500 & 812.37 & 111.23 & 2.12 \\
T5-large-2-gpt2-1-layers & 100 & 805.28 & 75.01 & 0.25 \\
T5-large-2-gpt2-1-layers & 500 & 805.28 & 102.17 & 1.28 \\
\hline
\end{tabular}
}
\caption{Efficiency metrics}
\label{tab:accents}
\end{table}

\begin{table}[h]
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{llll}
\hline
\textbf{Model(s)}                           & \textbf{En-Fr}      & \textbf{En-De}       & \textbf{En-Ro}      \\ 
\hline
T5-large-2-T5-small                         & 39.22 & 28.36 & 27.04         \\ 
T5-large-2-GPT2-small                       & 39.01 & 28.27 & 25.86         \\ 
\hline
T5-large-2-T5-small-Projector-Only          & \textbf{39.22} (1k, same after 50k) & \textbf{27.94} & \textbf{27.15}           \\
T5-large-2-GPT2-small-Original-Tokenizer    & \textbf{38.66} & \textbf{27.54} & \textbf{24.93}           \\
\hline
T5-Small-LoRA                               & 36.36 & 25.99 & 25.83         \\
T5-Small-Prefix-Tuning                      & 35.34 & 24.91 & 24.68         \\ 
T5-Small-Prompt-Tuning                      & 36.06 & 24.74 & 24.95         \\ 
\hline
\end{tabular}
\end{adjustbox}
\caption{Ablations for Translation}
\label{your_label_here}
\end{table}


\begin{table}
\centering
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lllll}
\hline
\textbf{Model(s)} & ROUGE-1 & ROUGE-2 & ROUGE-L & ROUGE-LSum\\
\hline
T5-large (zero-shot) & 40.07 & 18.84 & 28.82 & 37.30 \\
\hline
\hline
GPT2-small & 38.58 & 17.56 & 27.36 & 36.06 \\
GPT2-XL & 40.47 & 19.09 & 28.9 & 37.94 \\ \hline
T5-large-2-GPT2-small & 40.22 & 18.64 & 28.80 & 37.64\\
T5-large-2-GPT2-small-Original-Tokenizer & 40.65 & 19.29 & 29.36 & 38.15 \\
T5-large-2-GPT2-small-Projector-Only & 32.87 & 14.40 & 25.13 & 30.41 \\ \hline
GPT2-small-LoRA & 33.45 & 13.32 & 20.27 & 30.86 \\
GPT2-small-Prefix-Tuning & 32.61 & 12.68 & 19.62 & 30.04 \\
GPT2-small-Prompt-Tuning & 30.24 & 10.68 & 17.65 & 27.61 \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Ablations for Summarization}
\label{tab:accents}
\end{table}

\begin{table*}[t]
\begin{center}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c}
\hline
\textbf{model}                              & \textbf{coding} & \textbf{extraction} & \textbf{humanities} & \textbf{math} & \textbf{reasoning} & \textbf{roleplay} & \textbf{stem} & \textbf{writing} & \textbf{avg}    \\ \hline
\textbf{flan-alpaca-xxl  (zero-shot)}       & 1               & 4.1                 & 3.4                 & 1.1           & 2.7                & 4                 & 3.6           & 5.3              & 3.15            \\ \hline
\textbf{llama-13b (zero-shot)}                                         &     1.1 &         2.5 &        3.35 &  1.05 &       2.55 &      4.05 &  2.55 &      3.7 &  2.60625 \\ \hline
\textbf{flan-t5-xxl   (zero-shot)}          & 1               & 3.2                 & 1.6                 & 2.1           & 3.1                & 2.7               & 2.5           & 2.9              & 2.3875          \\ \hline
\rowcolor[HTML]{DAE8FC} 
\textbf{flan-alpaca-xxl-to-flan-t5-base-gt} & \textbf{1.6}    & \textbf{1.6}        & \textbf{2.4}        & \textbf{1.1}  & \textbf{1.8}       & \textbf{3.5}      & \textbf{2.5}  & \textbf{4}       & \textbf{2.3125} \\ \hline
\rowcolor[HTML]{DAE8FC} 
\textbf{flan-t5-base-gt}                    & \textbf{1}      & \textbf{1}          & \textbf{2.7}        & \textbf{1}    & \textbf{1.4}       & \textbf{2.6}      & \textbf{2.1}  & \textbf{3.9}     & \textbf{1.9625} \\ \hline
\textbf{flan-alpaca-base (zero-shot)}       & 1               & 1                   & 1.1                 & 1             & 2.5                & 2.9               & 2.1           & 2.9              & 1.8125          \\ \hline
\rowcolor[HTML]{DAE8FC} 
\textbf{gpt2-gt}                            & \textbf{1.1}    & \textbf{1}          & \textbf{2}          & \textbf{1}    & \textbf{2}         & \textbf{1.4}      & \textbf{1.9}  & \textbf{1.8}     & \textbf{1.525}  \\ \hline
\rowcolor[HTML]{DAE8FC} 
\textbf{flan-alpaca-xxl-to-gpt2-gt}         & \textbf{1}      & \textbf{1}          & \textbf{1.6}        & \textbf{1}    & \textbf{1.8}       & \textbf{1.7}      & \textbf{1.4}  & \textbf{2.7}     & \textbf{1.525}  \\ \hline
\textbf{flan-t5-base   (zero-shot)}         & 1               & 1.6                 & 1.3                 & 1.6           & 1.2                & 1.4               & 1.2           & 1.1              & 1.3             \\ \hline
\textbf{gpt2   (zero-shot)}                 & 1               & 1                   & 1                   & 1             & 1                  & 1.3               & 1             & 1.3              & 1.075           \\ \hline
\end{tabular}
\end{adjustbox}
\caption{MT Bench Results}
\end{center}
\end{table*}





\section{Tables used in presentation}

